Cooperative Modular Manipulation with Numerous Cable-Driven Robots for Assistive Construction and Gap Crossing

Soldiers in the field often need to cross negative obstacles, such as rivers or canyons, to reach goals or safety. Military gap crossing involves on-site temporary bridges construction. However, this procedure is conducted with dangerous, time and labor intensive operations, and specialized machinery. We envision a scalable robotic solution inspired by advancements in force-controlled and Cable Driven Parallel Robots (CDPRs); this solution can address the challenges inherent in this transportation problem, achieving fast, efficient, and safe deployment and field operations. We introduce the embodied vision in Co3MaNDR, a solution to the military gap crossing problem, a distributed robot consisting of several modules simultaneously pulling on a central payload, controlling the cables' tensions to achieve complex objectives, such as precise trajectory tracking or force amplification. Hardware experiments demonstrate teleoperation of a payload, trajectory following, and the sensing and amplification of operators' applied physical forces during slow operations. An operator was shown to manipulate a 27.2 kg (60 lb) payload with an average force utilization of 14.5\% of its weight. Results indicate that the system can be scaled up to heavier payloads without compromising performance or introducing superfluous complexity. This research lays a foundation to expand CDPR technology to uncoordinated and unstable mobile platforms in unknown environments.

==> Backups/BACKUP_01-27-24.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %2345678901234567890123456789012345678901234567890123456789012345678901234567890
% %        1         2         3         4         5         6         7         8


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%% SETUP Document %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out if you need a4paper

% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper

% \IEEEoverridecommandlockouts                              % This command is only needed if 
%                                                           % you want to use the \thanks command

% \overrideIEEEmargins                                      % Needed to meet printer requirements.

% % \usepackage{subfiles} % Best loaded last in the preamble
% % \subfile{utils}

% %In case you encounter the following error:
% %Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
% %Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
% %This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
% %Please use one of the alternatives below to circumvent this error by uncommenting one or the other
% %\pdfobjcompresslevel=0
% %\pdfminorversion=4

% % See the \addtolength command later in the file to balance the column lengths
% % on the last page of the document

% % The following packages can be found on http:\\www.ctan.org
% %\usepackage{graphics} % for pdf, bitmapped graphics files
% %\usepackage{epsfig} % for postscript graphics files
% %\usepackage{mathptmx} % assumes new font selection scheme installed
% %\usepackage{times} % assumes new font selection scheme installed
% %\usepackage{amsmath} % assumes amsmath package installed
% %\usepackage{amssymb}  % assumes amsmath package installed

% \include{Misc/Utils}

% \usepackage{amsmath}
% \usepackage[long]{optidef}
% \usepackage{mathtools}% http://ctan.org/pkg/mathtools
% \usepackage{ragged2e}
% \usepackage{tabularx}
% % \usepackage[showframe]{geometry}% http://ctan.org/pkg/geometry
% \usepackage{lipsum}% http://ctan.org/pkg/lipsum
% \usepackage[noadjust]{cite}


% \usepackage{draftwatermark}
% \SetWatermarkText{DRAFT}
% \SetWatermarkScale{1}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%% Start Document %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{document}
% \pagenumbering{Roman}


% % =======================================================================
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% title %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % =======================================================================
% \title{\LARGE \bf
% Assistive Construction with Cooperative Modular Manipulation with Numerous Cable-Driven Robots for Gap Crossing}

% \author{Kevin Murphy\inst{1,2} \and Joao C. V. Soares\inst{1,3} \and Justin Yim\inst{1} \and Dustin Nottage \inst{2} \and Ahmet Soylemezoglu \inst{2} \and  Joao Ramos\inst{1}% <-this % stops a space
% \thanks{*This work was supported by the US Army Corps of Engineers Engineering Research and Development Center - CERL via award number W9132T22C0013}% <-this % stops a space
% \thanks{$^1$Department of Mechanical Science and Engineering at the University of Illinois at Urbana-Champaign, USA}
% \thanks{$^2$ US Army Corps of Engineers Construction Engineering Research Laboratory, Champaign, IL 61822, USA}
% \thanks{$^3$ Dynamic Legged Systems Laboratory, Istituto Italiano di Tecnologia (IIT), Genova, Italy}
% % \thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
% %         Dayton, OH 45435, USA
% %         {\tt\small b.d.researcher@ieee.org}}%
% }

% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}

% % =======================================================================
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Abstract %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % 
% %To improve efficiency and safety in hazardous military gap-crossing operations, this research proposes a robotic solution can be adopted if it exhibits the following: modularity, scalability, physical reconfigurability, and force control.=======================================================================
% \begin{abstract}\\% start with problem. 
% When soldiers need to cross an obstacle such as a river or canyon, they need to construct and deploy a bridge on site. However, this procedure is conducted with dangerous, time and labor intensive operations, and specialized machinery. The authors envision that a scalable robotic solution can address the challenges inherent in the transportation problem, achieving fast, efficient, and safe deployment and field operations. 

% To this extent, the authors introduce Co3MaNDR, a system consisting of several modular robots simultaneously pulling on a central payload, controlling the cables' tensions to achieve a high level goal. Hardware experiments demonstrate teleoperation of a payload, trajectory following, and the sensing and amplification of operators' applied physical forces during slow operations. An operator was shown to manipulate an 80 lb payload with an average force utilization of 14.5\% of its weight. Results indicate that the system can be scaled up to heavier payloads without compromising performance. 

% \end{abstract}


% % =======================================================================
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Intro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % =======================================================================
% \section{Introduction}
% % Overview 
% Military gap crossing involves on-site construction of temporary bridges to overcome negative obstacles and increase field unit mobility and safety. Emplacing bridges allows rapid, efficient deployment and maintenance of supply lines supporting the movement of troops and equipment during combat operations. While beneficial, military bridging comprises several formidable challenges. 

% \red{\cite{hui2017} \cite{Thanapisudwong2018} \cite{connor2000} - military bridging citations.}

% Current methods require 1) assembly of bridging components using specialized vehicles and heavy equipment, which introduces 2) complex logistics for acquiring, transporting and deploying the necessary equipment and heavily trained operators. Using 3) copious time and hazardous manual labor, construction proceeds section by section on rollers, facilitating movement into final locations over obstacle areas. Harsh field conditions, like swamps, aquatic areas, or austere terrains, add challenges for accommodating heavy machinery and personnel. Danger is only increased in contested zones.

% Future military bridging requires a system with the flexibility to manipulate diverse bridges and components, operate in close proximity to humans, and provide a large workspace for effective operations. Meeting these capabilities will enhance the efficiency and effectiveness of field gap crossing, ensuring safety, and boost flexibility and capabilities for field units in diverse operational environments.

% This project overcame these challenges and pioneered a viable method which enables a lone person to install gap crossing solutions without heavy equipment. Our research introduces a modular robotic manipulation system (depicted in Fig. \ref{fig:entire_system}), where multiple robots independently act as force sources on a central payload, providing versatile solutions for large payload manipulation bridging, civil, and industrial sectors.
% % \vspace{-5mm}
% % \section{Introduction}
% % % Overview 
% % Military gap crossing involves on-site construction of temporary bridges to overcome negative obstacles and increase field unit mobility and safety. Emplacing bridges allows rapid, efficient deployment and maintenance of supply lines supporting the movement of troops and equipment during combat operations. While beneficial, military bridging comprises formidable challenges due to: 1) large personnel requirement, 2) inherently dangerous assembly tasks, and  3) complex logistics involved in acquiring, transporting and deploying the necessary equipment, especially in remote or hostile environments. 

% % This project aims to overcome these challenges, enabling a lone person to install gap crossing solutions without heavy equipment. Our research introduces a modular robotic manipulation system (depicted in Fig. \ref{fig:entire_system}), where multiple robots independently act as force sources on a central payload, providing versatile solutions for large payload manipulation bridging, civil, and industrial sectors.

% % \subsection{Military Bridging}
% % % Challenges and limitations and % Current Approaches 
% % Current methods involve transporting bridging components to the installation site followed by staging and assembly employing specialized vehicles, heavy equipment, large amounts of hazardous manual labor and time. During construction, bridges are constructed section by section on top of rollers. These rollers facilitate moving the completed sections and the full bridge into final locations over the obstacle area. Harsh field conditions, such as swamps, aquatic areas, or austere terrains, often pose additional difficulties for accommodating heavy machinery. Danger is only increased in contested environments.

% % Future military bridging necessitates the development of capabilities that address key requirements. The system should possess the flexibility to manipulate various types of bridges and components, be capable of operating in close proximity to humans. Additionally, a large workspace is crucial to accommodate the bridging operations effectively. By meeting these capabilities, future military bridging systems will significantly enhance the efficiency and effectiveness of bridging operations in diverse operational environments, protect human life, and increase flexibility and capabilities of field units. 

% \begin{center}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.485\textwidth]{Figs/gradient_V2.png}
% \caption{Co3MaNDR System, consisting of 4 modules (orange box) in planar configuration. The experimental setup (left) and CAD model (right) are shown overlayed onto each other, with an example payload (center).  } 
% \label{fig:entire_system}
% \vspace{-7mm}
% \end{figure}
% \end{center}
% \vspace{-10mm}

% \subsection{Related Works}
% Co3MaNDR combines several technologies in novel ways, so its formulation introduces diverse fields. 

% \red{Why havent other people doing this?}
% \red{bridging ref from proposal.}
% %https://www.youtube.com/watch?v=-8HSHOzbgzE&ab_channel=MabeyBridge


% \blue{cameras to control \cite{DALLEJ2019}, \cite{zake2019}}
% \blue{position control with MPC \cite{CDPR_MPC}}%this is 

% \subsubsection{\textbf{Force Control}}
% Instead of position or velocity control traditionally seen in robotics, force control is a strategy that focuses on regulating the forces exerted by robotic actuators during interactions throughout the completion of high level tasks. The MIT mini cheetah \cite{cheetah}, Boston Dyanamics' Spot \cite{BD_spot} and Atlas \cite{BD_atlas}, LIMS2-Ambidex \cite{limsII}, are all examples of force controlled robots. 

% % Force control is limited by the hardware being employed \citethis{idk man}. There are two main camps of electric actuators used for force control. Proprioceptive Actuators are characterized by their small gear ratios, which reduced non-linearities in the current-torque relationship and increase force transparency. While they have comparatively low sustained torque capabilities, they have high mechanical bandwidth. Series Elastic Actuators (SEAs) on the other hand, consist of a motor powering higher geared transmission with a spring connecting the transmission to the actuator output \citethis{}. While they have much higher sustained force capabilities, they exhibit low mechanical bandwidth. Both types have been shown to be capable of force control \citethis{stuff}. This project prioritized high mechanical bandwidth and utilized proprioceptive actuators. 
% Force control is limited by the hardware being employed. There are two main camps of electric actuators used for force control. Proprioceptive Actuators and Series Elastic Actuators (SEAs) have both been shown to be capable of force control and have their individual advantages and disadvantages\cite{proprio,cheetah,SEA}. This project prioritized high mechanical bandwidth and utilized proprioceptive actuators.


% \subsubsection{\textbf{Cable-Driven Parallel Robots}}

% % CDPR Overview 
% Cable-Driven Parallel Robots (CDPRs) are a class of robotic systems characterized by controlling an end-effector with parallel cable-based mechanisms. As CDPRs generally consist of stationary winches surrounding the workspace connected to the end effector with cables. Therefore CDPRs do not move serial components or the motors themselves, resulting in inertial effects being primarily caused by the payload. CDPRs are lightweight and have high payload-to-mass ratios compared to traditional robotic manipulators \cite{CDPR_survey}. While CDPRs are known for their adaptability and reconfigurability, they experience unique control challenges such as cable intersections limiting rotations, cables' inability to push, cable stretch and sag \cite{sag}. CDPR have been seen in a vast array of applications, including flight simulation \cite{helicopter}, construction and cinema\cite{CDPR_survey}, logistics \cite{FASTKIT}, marine platforms \cite{HOROUB2018314}, painting \cite{SERIANI20151}, rehabilitation \cite{ABBASNEJAD20161}, motion simulation \cite{SCHENK2018161}, additive manufacturing \cite{3D_print}, etc. 

% % Nature is appropriate for this 
% The nature of CDPRs lends itself to project requirements. CDPR’s actuators distributed around the workspace suggests distributing the robot as modular payloads onto several platforms or the environment. Module placement is a design choice; the system can easily reconfigure the placement and interaction of modules to match situational requirements. Similarly, scaling the number of modules allows scaling the total system lifting capabilities, making the system payload agnostic. Finally, CDPRs customarily cover expansive workspaces while maintaining dexterity and accuracy, which has been aligns with construction requirements. 

% % Why innapropriate 
% However, traditional CDPRs cannot act as a solution for the field construction problem. First, CDPRs generally utilize position control on a system with highly geared actuators, which preclude force control. Second, CDPRs almost always are based off of rigid separate structures surrounding the workspace, which increases the problems associated with field construction and transportation. Closed-loop force feedback has been shown in CDPR systems \cite{closed_loop_force_control}, but operations are limited by the physical hardware employed. 

% \subsubsection{\textbf{Multi-Agent Manipulation}}
% Multiple agents connected to the same rigid body creates closed kinematic chains, greatly increasing the complexity of the control problem. Multi-Agent Manipulation is exceptionally challenging for traditional robotics, such as highly geared industrial arms. Frictional effects increases non-linearly and rotor inertia is amplified by the square of the gear ratio \cite{youngwoo , youngwoo_b}, making actuators with large gear ratios non-backdrivable. In such systems, small pose errors cause substantial interaction forces which can damage the robots and the payload. 

% % Why innapropriate  
% Heavily controlled motions have be achieved \cite{bimanual}, but extremely slowly in disturbance free, known, and controlled environments. Manipulating deformable payloads \cite{deform_a, deform_b} circumvents issues with kinematic error. However, the specialized flexible payload are not matched to construction or structures. These solutions are ill-fitted for field operations. 

% An exciting project seen in \cite{Lynch} shows an SEA and omni-wheel based distributed robotic system that also shows human guided force amplification. However, this system is limited by the required controlled flat ground, the mobile module's footprint, and rigid parallel linkage connections reducing the range of motion of the payload.  













% \subsection{Approach and Contributions}
% This work proposes field bridging and other cumbersome payload manipulation can be achieved with Cooperative Mobile and Modular Manipulation with Numerous cable-Driven Robots (Co3MaNDR), a system engineered around a set of critical system attributes: modular robots distributed to support physical reconfigurability, compliant, backdrivability, and force control. 

% Co3MaNDR's approach shifted several paradigms, which informed system level design, dictated actuator and sensor selection, and structured the chosen control method. First, this approach replaces conventional employment of specialized heavy equipment with distributed, smaller collaborative modular robots. Co3MaNDR adopts a payload-centric controller based on interaction forces, deviating from the traditional position control methods employed in CDPRs and allowing system level force sensing and motions guided by operators physically applying force. Individual modules plan together as a single unit, but can act independently without coordination, increasing agility and adaptability in dynamic field environments. The variable number of modules, optimization-based control methods are particularly applicable. This innovative approach leverages the inherent advantages of distributed modular robotics and aligns seamlessly with the CDPR-based system design and introduces new capabilities.

% The authors designed and implemented this novel system design that is scalable, demonstrating operations with two to four novel modular robots, suggesting that heavier payloads can be manipulated by adding more modules. Design and implementation of a wrench-based controller draws its inspiration from the realm of force-controlled legged robotics. To the authors' knowledge, this is the first application of such proven control methods and hardware to Cable Driven Parallel Robots. Finally, validation of assumptions and functionality are experimental shown. The system was shown to lift an \red{80 lb} payload and with the operator exerting an average of 18.7\% of the payload's weight to control its motion. This novel system offers significant advancements in the field of robotics, enabling safe, efficient, and adaptable manipulation of heavy payloads in diverse and dynamic environments.



% % =====================================================================================================
% % =====================================================================================================
% % =====================================================================================================


























% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Methodology}
% \vspace{-5mm}
% \begin{center}
% \begin{figure*}[t]
%     \centering
%     % \includegraphics[width=\textwidth]{Figs/module_combined_V2.png}
%     \includegraphics[width=\textwidth]{Figs/Models_combined_V5.PNG}
% \caption{(a) System level dynamics diagram containing four modules (1,2,3,n) manipulating a generic payload. The generic number of modules are represented as simplified single module dynamics models(b). These are color coordinated with the Robotic Module CAD model (c). The upper assembly measures tension output direction (yaw, pitch, and roll). The lower assembly moves up and down on rails ensuring that the measured cable tension is solely from the vertical component of the cable.}
% \label{fig:module}
% \vspace{-7mm}
% \end{figure*}
% \end{center}

% \subsection{Scalable Force Based Controller}
% A crucial aspect of Co3MaNDR's innovative approach lies in holistically incorporating force control its design. This approach draws inspiration from the realm of force-controlled legged robotics\cite{QP_1,QP_2}, bringing these proven control methods and hardware into CDPRs. By synergistically combining these diverse subfields, Co3MaNDR's controller deviates from the traditional cable positions/lengths control and exclusively regulates forces between the modules and collective payload.









% The adoption of force control brings forth several compelling advantages. Firstly, it enables the monitoring and precise control of interaction forces, facilitating the sensing and recognition of external forces. This capability is instrumental in detecting and comprehending external forces resulting from collisions with unknown objects, people, or environmental entities at the system level. Constructing the controller to recognize and adapt to these external forces significantly enhances the safety of humans, other equipment, and the surrounding environment when operating in close proximity to Co3MaNDR.

% Moreover, force sensing introduces an invaluable dimension for human-robot interaction. The system can now detect and respond to applied forces with minimal resistance, allowing humans to physically guide the payload in a behavior referred to as force amplification. This human-in-the-loop approach can not only empower operators with a more intuitive and responsive means of control, but can also open the door to use the Co3MaNDR in widespread applications.

% % \begin{center}
% % \begin{figure}[b]
% %     \centering
% %     \includegraphics[width=0.485\textwidth ]{Figs/potato_w_modules_v1.png}
% % \caption{System level dynamics diagram containing four modules (1,2,3,n) manipulating a generic payload. Variable definition for equations listed. } 
% % \label{fig:potato}
% % \end{figure}
% % \end{center}

% Finally, by incorporating force control, Co3MaNDR eliminates the need for complex forward or inverse kinematics calculations, bypassing the resource-intensive typical path planning. This streamlined approach reduces the system's computational overhead and enhances real-time responsiveness and adaptability.

% \subsubsection{\textbf{Implemented Controller}}
% The payload-centric force controller is designed to control the net wrench acting on the payload. This controller takes in the current system state and desired payload wrench and determines the correct tensions to be applied to the payload by each module. The desired wrench, $W_des$, can be determined through various means, including teleoperation commands, gravity compensation, or a desired Cartesian payload position.
% \vspace{-1mm}
% \begin{equation}
% % W_{des} = [F_{x,des}, F_{y,des}, F_{z,des}, M_{x,des}, M_{y,des}, M_{z,des}]
% W_{des} = [F_{x}, F_{y}, F_{z}, M_{x}, M_{y}, M_{z}]_{des}
% \end{equation}

% The net wrench applied is determined from the Jacobian, which is a function of the ith tension unit vectors, $u_i$, and the reaching from the Center of Mass to the ith cable’s connection point, $r_i$. The Tension vector, $T$, is a column vector of all applied tension magnitudes. Fig. \ref{fig:module} shows labeled entities in a system level diagram. 
% \vspace{-2mm}
% \begin{equation}
% W_{applied}  = F = J T = 
%           \begin{bmatrix}
%           u_1, \dots, u_n\\
%           r_1 \times u_1, \dots, r_n \times u_n
%           \end{bmatrix} 
%           \begin{bmatrix}
%            T_{1} \\
%            \vdots \\
%            T_{n}
%          \end{bmatrix}
% \end{equation}

% Since cables cannot push and can only pull, most CDPR systems utilize more cables than number of Degrees of Freedom (DoF) being controlled, creating an over-constrained the system and expanding the solution set to be infinitely large. To navigate this complexity, this controller relies on quadratic programming (QP) optimization, which finds the decision vector (in this case the Tension vector, $T$) that minimizes the cost function within a set of linear constraints. Co3MaNDR’s cost function, mathematically shown in  Eq. \ref{eqn:cost_func}, is formulated to impose a weighted penalty for any deviation between the desired and achieved net payload wrench, while keeping tensions between minimum and maximum bounds.
% \vspace*{-1mm}
% \begin{mini}
%       {T}{\smashoperator{\sum_{\tab \tab \tab i \in \{X,Y,Z,\theta_x,\theta_y,\theta_z\} }} W_i (F_{i,des}-F_{i})^2 + W_T \smashoperator{\sum_{\tab j = 1,\dots,n}}T_j^2}{}{}
%       \addConstraint{AT \leq b}{}{}
%       \label{eqn:cost_func}
% \end{mini}

% % \begin{mini}
% %       {T}{\smashoperator{\sum_{\tab\tab i=[X,Y,Z,\theta_x,\theta_y,\theta_z]}{ W_i (F_{i,des}-F_{i})^2}} 
% %       + W_T \smashoperator{\sum_{j = 1,\dots,n}{T_j^2}}}{}{}
% %       \addConstraint{AT \leq b, }{\tab A\epsilon\Re^{2n,2n}, }{\tab b\epsilon\Re^{2n,1}}
% % \end{mini}
% % \begin{mini}
% %       {T}{\smashoperator{\sum_{\tab\tab i=[X,Y,Z,\theta_x,\theta_y,\theta_z ]}} W_i (F_{i,des}-F_{i})^2 + W_T \smashoperator{\sum_{j = 1,\dots,n}T_j^2}}{}{}
% %       \addConstraint{AT \leq b, }{\tab A\epsilon\Re^{2n,2n}, }{\tab b\epsilon\Re^{2n,1}}
% % \end{mini}
% % \begin{mini}
% %       {T}{\sum_{i=[X,Y,Z,\theta_x,\theta_y,\theta_z ]} W_i (F_{i,des}-F_{i})^2 + W_T \sum_{j = 1,\dots,n}T_j^2}{}{}
% %       \addConstraint{AT \leq b, }{\tab A\epsilon\Re^{2n,2n}, }{\tab b\epsilon\Re^{2n,1},}
% % \end{mini}
% % \begin{mini}
% %       {T}{\sum W_i (F_{i,des}-F_{i,appl})^2 + }{}{}
% %       \breakObjective{ W_T \sum_{j = 1,\dots,n}(T_j^2)}{}{} 
% %       \addConstraint{AT \leq b}{}{}
% %       i=[X,Y,Z,\theta_x,\theta_y,\theta_z ]
% % \end{mini}
% % \begin{mini}
% %       {T}{C(T) = W_x (F_{x,des}-F_{x,apl})^2 + }{}{}
% %       \breakObjective{W_y (F_{y,des} - F_{y,apl})^2 + }{}{} 
% %       \breakObjective{W_z (F_{z,des} - F_{z,apl})^2 + }{}{}
% %       \addConstraint{g(w_k)+h(w_k)}{=0,}{k=0,\ldots,N-1}
% %       \addConstraint{l(w_k)}{=5u,\quad}{k=0,\ldots,N-1}
% % \end{mini}
% % \begin{equation}
% % \begin{aligned}
% % & \underset{x = T}{\text{minimize}} \tab C(\dots) = W_x (F_{x,des}-F_{x,apl})^2 + 
% % & W_y (F_{y,des} - F_{y,apl})^2 + \\
% % & W_z (F_{z,des} - F_{z,apl})^2 + \\
% % & W_T \sum(T_i^2) + \\
% % & \text{subject to}
% % & & Ax \leq b \; i = 1, \ldots, m.
% % \end{aligned}
% % \end{equation}
% % Minimize C() = Wx*(Fx_des – Fx)^2 + Fy + Fz + W_t()^2 … 
% % •	T = T-I [1,…n] 
% % Subject to 
% % 

% $F_{i,des}$ and $W_i$ are the desired forces and weights respectively for the Cartesian position in the ith directions. $W_t$ is the tensions weight, which is added to spread the forces between all cables and avoid over-utilizing any single module. Since this term of the optimization is not as important as controller accuracy, $W_t$ should be at least an order of magnitude less than the Cartesian force weights. All weights were found experimentally. 

% This cost function has an analog analytic representation fitting standard QP formulation, where x is the decision vector (tensions). P, a positive definite matrix, and q, a matrix containing the linear terms in the formulation, are functions of the desired wrench and unit vectors. The matrices A and B are populated to keep tensions between minimum and maximum values.
% % \begin{equation}
% % C(P,q) = \frac{1}{2} x^T P x + q^T x
% % % P \in \mathbb{R}^{n,n}, \tab q \in \mathbb{R}^{1,n}
% % \end{equation}
% \vspace{-2mm}
% \begin{mini}
%       {T}{C(P,q) = \frac{1}{2} x^T P x + q^T x}{}{}
%       \addConstraint{AT \leq b,}{A\in\mathbb{R}^{2n \times 2n},}{b\in\mathbb{R}^{2n \times 1}}
%       \label{eqn:QP_rep}
% \end{mini}

% This formulation scales easily with changing the size of the decision vector and adding the additional force effects into the Q and P matrices. Consequently, the system level control effort scales effortlessly by adding or removing modules, facilitating Co3MaNDR adapting to varying operational demands. 

% \subsubsection{\textbf{Assumptions and Requirements}}
% While the controller outlined in this paper demonstrates an elegant and effective approach to robotic control, it is based on several underlying assumptions which relies on appropriate utilization.  

% First, the robot's actuators are assumed to function as pure torque sources, disregarding complexities like actuator dynamics, friction and stiction, damping, and inertial effects. This assumption is made viable through our deliberate choice of backdrivable actuators designed for compliant force control operations and utilizing systems within the operational regimes minimizing neglected effects.  

% Second, the controller assumes modules are rigidly connected to the environment, precluding any shifting or tipping. 

% Third, cables are assumed to be ideal (massless, infinitely stiff, no routing friction, …). This assumption is well-founded when using stiff cables that are light in comparison to the payload and tensions remain under plastic deformations limits. The neglected effects are orders of magnitude smaller that operational forces, which therefore dominate the system equation.

% Finally, the current implementation ignores dynamic effects and assumes the payload and modules do not experience dynamic abrupt motions. 

% % \begin{center}
% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[scale = 0.55 ]{Figs/draft 1/module.JPG}
% % \caption{Robotic Module. The upper assembly, which measures tension output direction. The lower assembly moves up and down on rails and directly measures cable tension.} 
% % \label{fig:module}
% % \end{figure}
% % \end{center}
% \vspace{-2mm}
% \subsection{Implementation}
% \subsubsection{\textbf{Module Design}}
% The robotic modules, seen in Fig. \ref{fig:module}, were engineered to support the assumptions in the controller, house all necessary components within a structurally robust, comparatively lightweight, and wide structure, and provide easy mounting to the operational environment. 

% The lower pulley assembly is mounted on linear rails (green) and firmly secured by a load cell (blue) to provide precise closed-force feedback. The height of the lower pulley can be adjusted to ensure that the cable runs perpendicular to the load cell's measurement axis and linear rails; this results in load cells solely measuring cable tension. 

% In the upper pulley assembly (red), three sets of encoders are incorporated to measure the cables' yaw, pulley roll, and measurement arm pitch; these characterize the applied tension unit vector.

% Finally, the separation of the motor and drum (purple) within the module, connected by toothed belts, offers flexibility in adjusting pulley ratios and tuning motor attributes such as speed, backdrivability, and torque capabilities, and enhances adaptability and the system.

% \begin{table}[t]
% \centering
% \caption{High level Bill of Materials for system with four modules} 
% \vspace{-3mm}
% \begin{tabularx}{3.3in}{|X|X|c|}\hline
% \textbf{Item} & \textbf{Use} & \textbf{Qty} \\
% \hline
% Laptop & Labview/control interface &  1 \\
% \hline
% Westwood Robotics PB02P & Main actuators &  4 \\
% \hline
% NI cRIO-9082 & System RT computer &  1 \\
% \hline
% NI 9205 Module& Analog input card&  1 \\
% \hline
% NI 9264 Module& Analog output card&  1 \\
% \hline
% NI 9403 Module& Digital IO card &  1 \\
% \hline
% NI 9871 Module& RS485 bus card &  1 \\
% \hline
% NI 9870 Module& RS232 bus card&  1 \\
% \hline
% NI 9381 Module& Multifunction I/O for cRIO &  1 \\
% \hline
% VectorNav VN-100 IMU & Estimate system pose &  5 \\
% \hline
% 4S LiPo Batteries & Main power for the system &  8 \\
% \hline
% 24V Kobalt Battery & Power sources for Load cells &  4 \\
% \hline
% Load Cells and Amplifiers & Closed loop force feedback &  4 \\
% \hline
% AEAT-6010-A06 Encoders & Measure angle state &  12 \\
% \hline
% Vicon Vero Motion Capture System & Closed loop position feedback - 8 cameras &  1 \\
% \hline
% \end{tabularx}
% \label{tab:BoM}
% \vspace{-6mm}
% \end{table}

% \subsubsection{\textbf{Hardware}}
% The experimental system consists of four modules. Fig. \ref{fig:flow_chart} shows a high-level flow diagram connecting components and Table \ref{tab:BoM} details them. Main control runs in real-time on an NI Compact Rio (cRIO) with expansion cards for analog input/output, RS485 and RS232 communication busses, and GPIO connections. All connections are connected with physical wiring between modules and the cRIO. Each module contains three 12-bit encoders, 1 IMU, 1 load cell/amplifier, and an actuator. 

% To support ideal cable assumptions, cables were selected to have minimal elongation, stay below 60\% load capacity during operations, and pre-stretched.

% \begin{center}
% \begin{figure}[b]
%     \vspace{-4mm}
%     \centering
%     \includegraphics[width=0.485\textwidth ]{Figs/system_control_diagram_w_fk_full_names.PNG}
%     \vspace{-7mm}
% \caption{System level control diagram for Co3MaNDR. Modules (red regions) contain individual $PID+I_{ff}$ loops, actuators, and sensors. The wrench based control loop (purple shaded region) shows the payload being controlled by any external wrench and applied tensions, converting from net wrench. The Cartesian control loop (light blue region) encapsulates the wrench loop and uses a pose $PID$ to regulate the desired wrench } 
% \label{fig:flow_chart}
% \end{figure}
% \end{center}


% \vspace{-6mm}
% \subsubsection{\textbf{System Level}}
% The system’s control diagram when given force commands is shown within the purple zone in Fig. \ref{fig:flow_chart}. Payload wrench commands produce desired cable tensions. These are fed into a PID layer, minimizing steady state error and adding closed loop force feedback. External wrenches ($W_{ext}$) applied by operators guiding motion are introduced directly to the plant as an external disturbance. The blue zone in \ref{fig:flow_chart} houses the Cartesian control loop. Here, the PID pose controller encapsulates positional commands and closed-loop pose feedback from forward kinematics and Vicon Vero Motion Capture system. 

% Rapid control rates have shown to be instrumental in force control robotics \cite{control_rate}. In implementation, the proposed QP controller converges and on average in 2ms and runs at 500Hz with feedback from IMUs and Vicon data at 200Hz and encoders at 1kHz. The lower level PID reads load cells and sends control commands tensions at 1kHz.

% \vspace{-1mm}
% \section{Experiments}
% \vspace{-1mm}
% A set of experiments was conducted to confirm the validity of assumptions in the system and controller design, verify that the prototyped system exhibits proposed requisite traits, and demonstrate scaled component manipulation capabilities. 

% \subsection{Experimental Setup}
% These experiments limit themselves to planar Cartesian position control with four modules. The Planar setup experimental consisted of stacking one module on top of another and rigidly mounting them on top of jersey barriers, considered immovable at the operational force scale. Two identical setups were constructed facing each other creating a 4x2.5m planar workspace. The number of modules can be changed to match the number of available modules, lift heavier loads, or match the environment. Similarly, the number of controlled DoF can be adjusted to achieve desired manipulation effects.

% \subsection{Module Characterization}
% The proposed control scheme is predicated on the assumption of ideal force sources. The first set of experiments characterizes module performance and ascertains to what degree they may be represented as a pure tension source. 

% In the initial phase of this experiment, we examine modules exerting force by rigidly connecting the module and cable to the environment. Starting from the minimum allowed torque, we command various steps in cable tension while recording the actual forces applied. The subsequent phase investigates the modules' ability to absorb forces, focusing on their level of backdrivability. This involves introducing error to a module assigned to maintain a constant tension.

% \subsection{Scaling and Modularity}
% The second experiment was designed to show exhibit control scaling, physical reconfiguration, and modularity attributes while exhibiting teleoperation and trajectory following abilities. 

% This experiment was subdivided into two parts. In each, the system moved the same payload in a prescribed trajectory; however, one experiment used two modules and one used four. The performance of each module and system as a whole was compared. 

% \subsection{Manipulation and Force Amplification}
% The final experiment was designed to show system compliance, force control, safe interactions, and effort amplification. It consisted of a human operator physically manipulating an object whose weight was compensated for by the system. The motion of the payload was recorded and compared to the measured and commanded tensions. 
% \vspace{-12mm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \vspace*{-\baselineskip}
% \begin{center}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.46\textwidth]{Figs/step_response.png}
%     \vspace{-4mm}
% \caption{Module characterization for step responses of several commanded tension magnitudes. Each experiment showed rise times < 0.7ms and settling times between 0.75-3.8 ms. Larger amplitude steps had large overshoots. In use, commanded tensions will not have large jumps, so performance in 50N step response is considered fitting and sufficient for operations.} 
% \label{fig:steps}
% \vspace{-5mm}
% \end{figure}
% \end{center}

% % \begin{center}
% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[scale = 0.15]{Figs/backdrive_tensions.jpeg}
% % \caption{Module characterization for back-driving during constant commanded tension} 
% % \label{fig:backdrive}
% % \end{figure}
% % \end{center}

% \begin{center}
% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.485\textwidth]{Figs/moving_traj.png}
%     \includegraphics[scale=0.55]{Figs/moving_traj_B.png}
%     \vspace{-4mm}
%     \caption{Co3MaNDR System following moving tension reference trajectory at several frequencies. Despite minimal lag and exhibited stiction stair-stepping effects, the desired force trajectory is followed closely.} 
% \label{fig:moving_traj}
% \vspace{-5mm}
% \end{figure}
% \end{center}

% % \begin{center}
% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[scale = 0.15]{Figs/backdrive_tension_vs_vel.jpeg}
% % \caption{Module characterization for back-driving during constant commanded tension} 
% % \label{fig:backdrive_ten_vs_vel}
% % \end{figure}
% % \end{center}
% % \begin{center}
% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[scale = 0.4]{figures/NAME.PNG}
% % \caption{} 
% % \label{fig:LABEL}
% % \end{figure}
% % \end{center}
% \section{Results and Discussion}
% \vspace{-8mm}
% % \includegraphics[scale = 0.75]{Figs/vel-tension_combined.png}
% \begin{center}
% \begin{figure*}[t]
%     \centering
%     % \includegraphics[width=\textwidth]{Figs/vel-tension_combined.png}
%         % \includegraphics[scale=1]{Figs/test.png}
%     \includegraphics[scale=0.5]{Figs/vel-tension_combined_B.png}
%     \vspace{-3mm}

% \caption{Module characterization for back-driving during constant commanded tension. Top left shows that the tension error stays within the same range despite tension magnitude. Bottom left show the velocity of the cable, exhibiting stiction behaviors. Right graph shows the tension error vs velocity relationship, finding a negative correlations between the two. Stiction is also depicted at $\pm$ 10N on the Y (Tension) axis}
% \vspace{-6mm}
% \label{fig:backdrive}
% \end{figure*}
% \end{center}
% \subsection{Module Characterization}
% % \vspace{-1mm}
% The module design encompasses friction minimization, but it cannot be completely eliminated. Friction most clearly expressed itself through non-uniform end-effector task-space inertia. Motion in directions opposite of the tension vectors ($\pm X$) backdrove the system’s total set of motors significantly further than motions that travelled orthogonal to them ($\pm Z$). Any backdriving displacement requires overcoming reflected inertia and motor damping. Moving the payload in X directions felt heavier while motions in the Z direction caused had smaller displacement and were manually moved quite easily. Testing without the closed loop tension sensing confirmed and accentuated these results.

% \subsubsection{\textbf{Exerting Forces}}
% To verify modules as pure torque output sources, Fig. \ref{fig:moving_traj} compares desired and measured tension from a module commanded sinusoidal trajectories. Stiction is seen in the stair-stepping effect, smaller adjustments in tension and motor motion. The small error in the tension profile following in comparison to the tension magnitude, so is viewed as disturbance.

% Fig. \ref{fig:steps} shows step responses of the four magnitudes. Average human response times are 250-400ms including sensing, deciding, planning, and beginning the action \cite{neuro}. Rise times are universally within 75 ms, Co3MaNDR system is sufficiently fast to mimic manual assembly operations. The overshoot seen in the larger steps is a product of the feed forward current and PID controller compounding efforts at the initial command. While the overshoot can cause large oscillations and instability with large steps, the smallest step has virtually no overshoot and settling time under 100ms. Tension trajectories during several experiments seen in Fig \ref{fig:ten_mag_compare}, show that the changes in operational commanded tension do not approach 50N step. As Co3MaNDR is used in relatively slow operations, operational performance is skewed toward the lower magnitude steps responses and overshoot becomes a non-issue.


% \subsubsection{\textbf{Backdriving}}
% Fig. \ref{fig:backdrive} shows measured tension error and velocity during backdriving experiments. Stiction again presents itself in sharp motions around $\pm 10N$ of the read trajectories along zero velocity. The tests with zero commanded tension does not follow this trend due to the weight of the lower pulley assembly not being held up by the tensioned cable skewing the readings. 

% Interestingly, the magnitude of the tension error did not increase with higher exerted forces, showing disturbances do not scale with control effort. Results indicate that proprioceptive force controlled CDPRs can be scaled up to larger tensions without greatly increasing error. This supports the conclusion that the backdriving effects are unavoidable and not a control error. 

% These experiments  confirm that the modules successfully achieve force control and act as a pure torque source during motions within human manipulation speed regime. 




% \begin{center}
% \begin{figure}[h]
%     \centering
%     \vspace{-3.00mm} 
%     \includegraphics[width=0.485\textwidth]{Figs/compare_2_and_4_mod_motion.png}
%     \vspace{-7.00mm}
% \caption{Paths comparing the end-effector's motion during experiments with two and four module configurations. Motions are repeatable and comparable. Stiction is seen in zig-zagging in payload motion. } 
% \label{fig:motion_compare}
% \vspace{-3.00mm}
% \end{figure}
% \end{center}

% \vspace{-9.00mm}

% \subsection{Scaling and Modularity}
% The trajectory commanded and executed for several two and four module trials are shown in Fig. \ref{fig:motion_compare}, where both configurations achieved the desired macroscopic payload trajectory. The effects of static friction is seen in the trajectories as a series of linear motions connected by directional changes and temporal pauses. Fig \ref{fig:ten_mag_compare} shows the tension signals in both configurations in their comparable operations. Throughout experiments, the four module configuration's average magnitude was only half the tension when only using two. Additionally, the ratio absolute maximum tension achieved between the four to two module modes is ~75\%.

% Intuitively, the four module configuration spreads out the torque requirements to more modules, so used proportionally less of each module’s maximum torque capabilities. This not only is safer for the system, but it implies that more modules increase system lift capacity, which confirms scalable control on a physically reconfigurable modular system.  


% \subsection{Manipulation and Force Amplification}
% Fig. \ref{fig:measured_tension} shows both the payload weight and the measured forces the operator applied to the payload during interactive manipulation. The operator exerts an estimated maximum force of approximately 105.5N and average approximately \red{50N}, only \red{39.4\% and 18.7\% }of the payload’s total weight respectively. Overcoming the object’s inertia cannot practically be overcome through haptic sensing without adding instability to the system; therefore, it is considered a constant in this scenario. This result confirms the system achieves force control and compliance sufficient for interactive force amplification.
 
% % Excitingly, the tension needed to backdrive a module is close to the that needed to move a payload; this results suggest that the human’s externally applied forces go towards overcoming static friction in the system and accelerating the payload, but not counteracting gravity. Overcoming the object’s inertia cannot practically be overcome through haptic sensing without adding instability to the system; therefore, it is considered a constant in this scenario. This result confirms the system achieves force control and compliance sufficient for interactive force amplification.

% \begin{center}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.485\textwidth]{Figs/compare_2_and_4_mod_tensions.png}
%     \vspace{-7.00mm}
% \caption{ Each module's tension trajectories during two module experiments (top), four module experiments (middle), and their respective averages (bottom). Average tension in four module experiments is consistently half that of two module experiments showing scalability in control and capabilities, reconfiguability, and modalarity.} 
% \label{fig:ten_mag_compare}
% \end{figure}
% \end{center}

% \vspace{-4mm}

% \begin{center}
% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.485\textwidth]{Figs/payload_weight_vs_exerted_forces_param.png}
%     \includegraphics[scale=0.5]{Figs/payload_weight_vs_exerted_forces_param_B.png}
%     \vspace{-3mm}
% \caption{Forces human exerted on a payload supported by Co3MaNDR during force amplification and manual manipulation. Maximum and average effort is around \red{39.5}\% and \red{14.5}\% of the payloads weight respectively.} 
% \label{fig:measured_tension}
%     \vspace{-7mm}
% \end{figure}
% \end{center}


% \vspace{-15mm}
% \subsection{Limitations}
% \subsubsection{\textbf{Proportions and Scale}}
% The most obvious limitation of the system is the reduced lifting capacity compared to motors with traditionally high gear ratios. The prototype was designed and components chosen based off simulated values  performing bridging operations scaled down (for practicality) to moving a 30kg payload throughout the workspace. However, since the tension error magnitude was found to not scale with control effort, utilizing more massive payloads will make nonlinear frictional and backdriving effects proportionally smaller. 

% \subsubsection{\textbf{Actuator Balance}}
% SEAs, QDDs, hydraulic, or other types of actuators can be implemented for a full-scale design. Introducing larger friction will greatly reduce system capabilities. It will also increase the antagonistic forces between modules and that operator manual guidance must overcome. Increasing the transparency and torque capacity of the system can grant significantly larger force multiplication, allowing the same person to manipulate a comparatively more massive payload in the same manner. Determining the best actuation method is a balancing act considering the utility and effects of backdrivablity, mechanical bandwidth, sustained and burst torque capabilities, friction, etc.

% \subsubsection{\textbf{Controlling Pose}}
% Manipulating objects's  spatial position is useful; however, bridging, construction, and other applications requires controlling the position and orientation of the payload. CDPRs are generally over-constrained due to cable’s ability to only pull and not push on its end-effector. The controller is designed to expand control  to additional DoF; external simulations confirmed the validityof this approach. However, controlling additional DoF also places limits on the possible number of modules, configurations, and feasible workspaces. 

% \subsubsection{\textbf{Operational Mobility}}
% These experiments utilize static modules, limiting their utility in the field. Transporting a massive payload using this approach would necessitate repeatedly setting up a workspace, moving the payload, and finally moving the workspace to an advanced position. While mobile CDPRs do exist \cite{FASTKIT,mcdpr}, they generally require specialized platforms moving in coordinated in ideal and well-known environments. Adding long distance field transportation capabilities to this technology increases potential mission capabilities in civil, industrial, and military scenarios. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Conclusion}
% % Statement of Purpose restated 
% To address the unique combination of challenges and limitations inherent in field current bridging techniques, this research proposed solutions must have the following attributes: modular, physically reconfigurable, scalable control, force controlled, and compliant. These attributes shaped the payload and platform agnostic Co3MaNDR system’s design and implementation.

% % Summarize Key Findings
% % Three types of experiments were conducted to confirm system functionality and validity of approach.
% % that force control is a viable approach in low speed operations,
% A set of experiments verified the viability of assumptions and showed the proposed system attributes. The first experiment included comparing torque output and absorption to ideal force control cases, finding that assumptions hold during slower operations. The second experiment exhibited system level modularity and reconfigurability by moving a 16kg  payload following the same trajectory with different number and configuration of individual robotic modules. Results showed that doubling the number of modules roughly reduced the average cable tension, indicating that system's maximum lifting capabilities and safety scales with the number of modules. Finally, the force a human operator applied to move a \red{80lb} payload in several directions during physical manipulation found to reach a maximum and average of \red{39.4\% and 18.7\%} of the payload’s total weight respectively. This force amplification interaction allowed one person to manipulate a large object with proportionally smaller forces. Since the tension error did not scale with tension magnitude, the results suggest that similar force multiplication can be conducted at a larger magnitude without greatly increasing tension error. 

% % Highlight Significance /Discuss Implications
% This technology has the potential to remove the need for heavy equipment in field construction operations, reducing logistical burdens, increasing environmental suitability, and vastly increasing transportation and construction speeds. Additionally, the system's proprioceptive nature can potentially improve operator safety during assembly and transportation operations. Adoption of this approach may reduce manual requisite manual labor and improve personnel safety. 

% % Future Blurb 
% Further work in this field will address the number of controlled DoFs, the mobility and coordination of modules, vision systems incorporated for field operations, and actuation limitations.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \section*{APPENDIX}

% % Appendixes should appear before the acknowledgment.

% % \section*{ACKNOWLEDGMENT}

% % The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % \begin{thebibliography}{99}
% %  % \include{refs.tex}
% % \bibitem{example} \red{DO BIB LATER 2023, ch. 1.}
% % % \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% % % \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% % % \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% % % \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% % % \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% % % \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% % % \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% % % \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 

% % % WE CAN ALSO USE A SEPERATE BIB FILE 
% % % \bibliography{refs.bib}
% % \end{thebibliography}

% \bibliographystyle{ieeetr}
% \bibliography{main}

% \end{document}


==> co3mandr_system_paper/Misc/Utils.tex <==
% Author: Kevin Murphy
% email: kevin.f.murphy14@gmail.com
% 
% This document is a collection of functions that I find useful for latex work. 
% it is included seperately for my happiness and cleanliness. 
% 
% use \include{utils} to call file in any supporting file  

% ======================================================================================================
%   ====== Function List ====== 
% * Colored text
%   -   Red
%   -   orange
%   -   Yellow
%   -   Green
%   -   Blue
% * Shrug emoticon 
% * tab
% ======================================================================================================


% ================================================ COLORS ============================================== 
\usepackage[x11names]{xcolor}
% \usepackage[dvipsnames]{xcolor}

% Define some macros for convenience
% TEXT
% https://tex.stackexchange.com/questions/141569/highlight-textcolor-and-boldface-simultaneously
% https://www.overleaf.com/learn/latex/Using_colours_in_LaTeX
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\white}[1]{\textcolor{white}{#1}}
\newcommand{\darkgray}[1]{\textcolor{darkgray}{#1}}
\newcommand{\lightgrey}[1]{\textcolor{lightgrey}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\lime}[1]{\textcolor{lime}{#1}}
\newcommand{\olive}[1]{\textcolor{olive}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\pink}[1]{\textcolor{pink}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\teal}[1]{\textcolor{teal}{#1}}
\newcommand{\violet}[1]{\textcolor{violet}{#1}}

% HIGHLIGHT
\usepackage{soul}
\DeclareRobustCommand{\hlred}[1]{{\sethlcolor{red}\hl{#1}}}
\DeclareRobustCommand{\hlgreen}[1]{{\sethlcolor{green}\hl{#1}}}
\DeclareRobustCommand{\hlblue}[1]{{\sethlcolor{blue}\hl{#1}}}
\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{cyan}\hl{#1}}}
\DeclareRobustCommand{\hlmagenta}[1]{{\sethlcolor{magenta}\hl{#1}}}
\DeclareRobustCommand{\hlyellow}[1]{{\sethlcolor{yellow}\hl{#1}}}
\DeclareRobustCommand{\hlblack}[1]{{\sethlcolor{black}\hl{#1}}}
\DeclareRobustCommand{\hlgray}[1]{{\sethlcolor{gray}\hl{#1}}}
\DeclareRobustCommand{\hlwhite}[1]{{\sethlcolor{white}\hl{#1}}}
\DeclareRobustCommand{\hldarkgray}[1]{{\sethlcolor{darkgray}\hl{#1}}}
\DeclareRobustCommand{\hllightgrey}[1]{{\sethlcolor{lightgrey}\hl{#1}}}
\DeclareRobustCommand{\hlbrown}[1]{{\sethlcolor{brown}\hl{#1}}}
\DeclareRobustCommand{\hllime}[1]{{\sethlcolor{lime}\hl{#1}}}
\DeclareRobustCommand{\hlolive}[1]{{\sethlcolor{olive}\hl{#1}}}
\DeclareRobustCommand{\hlorange}[1]{{\sethlcolor{orange}\hl{#1}}}
\DeclareRobustCommand{\hlpink}[1]{{\sethlcolor{pink}\hl{#1}}}
\DeclareRobustCommand{\hlpurple}[1]{{\sethlcolor{purple}\hl{#1}}}
\DeclareRobustCommand{\hlteal}[1]{{\sethlcolor{teal}\hl{#1}}}
\DeclareRobustCommand{\hlviolet}[1]{{\sethlcolor{violet}\hl{#1}}}

% ======================================================================================================

% ======================================================================================================
\newcommand{\DarkTheme}{\pagecolor{darkgray} \color{white}}
% ======================================================================================================


% =============================================== shruggie =============================================
\usepackage{graphicx}

\def\shrug{\texttt{\raisebox{0.75em}{\char`\_}\char`\\\char`\_\kern-0.5ex(\kern-0.25ex\raisebox{0.25ex}{\rotatebox{45}{\raisebox{-.75ex}"\kern-1.5ex\rotatebox{-90})}}\kern-0.5ex)\kern-0.5ex\char`\_/\raisebox{0.75em}{\char`\_}}}

\newcommand{\shruggies}[1]{
\tiny\shrug
\scriptsize\shrug
\footnotesize\shrug
\small\shrug
\normalsize\shrug
\large\shrug
\Large\shrug
\huge\shrug
\Huge\shrug
}

\newcommand{\shruggiesCol}[1]{
\tiny\shrug\\
\scriptsize\shrug\\
\footnotesize\shrug\\
\small\shrug\\
\normalsize\shrug\\
\large\shrug\\
\Large\shrug\\
\huge\shrug\\
\Huge\shrug\\
}
% ======================================================================================================

% ================================================= Tab ================================================
\newcommand\tab[1][5mm]{\hspace*{#1}}

% ======================================================================================================

% =====================================================================================================
\newcommand{\citethis}[1]{\textcolor{red}{[CITE]} }

% ======================================================================================================
\newcommand{\bM}{\mathbf}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\mat}[1]{\begin{matrix} #1 \end{matrix}}
\newcommand{\smat}[1]{\begin{smallmatrix} #1 \end{smallmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\bsmat}[1]{\begin{bsmallmatrix} #1 \end{bsmallmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\psmat}[1]{\begin{psmallmatrix} #1 \end{psmallmatrix}}





\newcommand{\inst}[1]{$^ {#1} $}

% ======================================================================================================
% ======================================================================================================

